Approximating the Minimum Equivalent Digraph

The MEG (minimum equivalent graph) problem is, given a directed graph, to find a small subset of the edges that maintains all reachability relations between nodes. The problem is NP-hard. This paper gives an approximation algorithm with performance guarantee of pi^2/6 ~ 1.64. The algorithm and its analysis are based on the simple idea of contracting long cycles. (This result is strengthened slightly in ``On strongly connected digraphs with bounded cycle length'' (1996).) The analysis applies directly to 2-Exchange, a simple ``local improvement'' algorithm, showing that its performance guarantee is 1.75.

==> contract.tex <==
\begin{picture}(0,0)%
\special{psfile=contract1.ps}%
\end{picture}%
\setlength{\unitlength}{0.012500in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(248,184)(58,631)
\put(275,705){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}active}}}
\put(240,755){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}active}}}
\put(195,802){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}root}}}
\put(213,644){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}inactive}}}
\put(187,681){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$W$}}}
\put(306,657){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}active}}}
\put(294,639){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$U$}}}
\put( 58,688){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}inactive}}}
\put( 85,748){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}inactive}}}
\put(138,667){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}inactive}}}
\end{picture}


==> cover-test.tex <==
\begin{picture}(0,0)%
\special{psfile=cover-test1.ps}%
\end{picture}%
\setlength{\unitlength}{0.012500in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(137,96)(99,684)
\put(121,702){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$v^+$}}}
\put(158,720){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$u^-$}}}
\put(212,709){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$v^+$}}}
\put(203,762){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$u^+$}}}
\put(157,767){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$x$}}}
\put(121,762){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$u^+$}}}
\put(135,740){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$v^-$}}}
\put(156,684){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$y$}}}
\end{picture}


==> exam.tex <==
\begin{picture}(0,0)%
\special{psfile=exam1.ps}%
\end{picture}%
\setlength{\unitlength}{0.012500in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(413,328)(62,460)
\put( 97,644){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}Graph G}}}
\put( 66,460){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}After traversing edge (7,6)}}}
\put(222,460){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}After traversing edge (6,8)}}}
\put(386,460){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}Edges in C}}}
\put(205,645){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}After traversing edge (3,1)}}}
\put(351,644){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}After traversing edge (6,4)}}}
\put(182,666){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}8}}}
\put(173,700){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}7}}}
\put(161,730){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}6}}}
\put(141,749){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}5}}}
\put(102,765){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}1}}}
\put( 95,748){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}2}}}
\put( 89,726){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}3}}}
\put( 80,700){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}4}}}
\put(326,665){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}8}}}
\put(316,699){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}7}}}
\put(304,730){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}6}}}
\put(284,749){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}5}}}
\put(255,771){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}1}}}
\put(241,750){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}2}}}
\put(235,725){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}3}}}
\put(234,706){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}4}}}
\put(474,666){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}8}}}
\put(464,700){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}7}}}
\put(451,736){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}6}}}
\put(429,766){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}5}}}
\put(402,775){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}1}}}
\put(390,748){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}2}}}
\put(385,730){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}3}}}
\put(385,710){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}4}}}
\put(100,532){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}4}}}
\put(101,555){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}3}}}
\put(107,574){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}2}}}
\put(121,600){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}1}}}
\put(147,591){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}5}}}
\put(168,561){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}6}}}
\put(198,512){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}7}}}
\put(203,478){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}8}}}
\put(357,479){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}8}}}
\put(352,513){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}7}}}
\put(322,561){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}6}}}
\put(302,592){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}5}}}
\put(275,600){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}1}}}
\put(256,555){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}3}}}
\put(256,534){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}4}}}
\put(264,577){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}2}}}
\put(475,495){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}8}}}
\put(466,528){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}7}}}
\put(455,558){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}6}}}
\put(434,578){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}5}}}
\put(394,593){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}1}}}
\put(387,575){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}2}}}
\put(381,554){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}3}}}
\put(377,526){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}4}}}
\end{picture}


==> lbound.tex <==
\begin{picture}(0,0)%
\special{psfile=lbound1.ps}%
\end{picture}%
\setlength{\unitlength}{0.012500in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(406,165)(73,640)
\end{picture}


==> lbound2.tex <==
\begin{picture}(0,0)%
\special{psfile=lbound21.ps}%
\end{picture}%
\setlength{\unitlength}{0.012500in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(303,120)(56,630)
\put(170,650){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}Edges returned by 2-Exchange}}}
\put(170,630){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}Edges not used by 2-Exchange}}}
\end{picture}


==> np.tex <==
\begin{picture}(0,0)%
\special{psfile=np1.ps}%
\end{picture}%
\setlength{\unitlength}{0.012500in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(399,232)(73,580)
\put(176,595){\makebox(0,0)[b]{\smash{\SetFigFont{10}{12.0}{rm}Variable gadget. Incoming edges from root,}}}
\put(179,580){\makebox(0,0)[b]{\smash{\SetFigFont{10}{12.0}{rm}outgoing edges to clause vertices.}}}
\put(113,799){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}Root}}}
\put(322,795){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}Root}}}
\put(205,612){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$+$}}}
\put(292,683){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$+$}}}
\put(291,748){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$-$}}}
\put(325,625){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$-$}}}
\put(408,617){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$+$}}}
\put(467,705){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$-$}}}
\put(432,774){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$+$}}}
\put(264,702){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$-$}}}
\put(230,772){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$+$}}}
\put( 73,692){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$+$}}}
\put( 88,752){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$-$}}}
\put(123,619){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}$-$}}}
\put(310,588){\makebox(0,0)[lb]{\smash{\SetFigFont{10}{12.0}{rm}Edges in SCSS for variable=TRUE.}}}
\end{picture}

